DVFL: A Vertical Federated Learning Method for Dynamic Data

Federated learning, which solves the problem of data island by connecting multiple computational devices into a decentralized system, has become a promising paradigm for privacy-preserving machine learning. This paper studies vertical federated learning (VFL), which tackles the scenarios where collaborating organizations share the same set of users but disjoint features. Contemporary VFL methods are mainly used in static scenarios where the active party and the passive party have all the data from the beginning and will not change. However, the data in real life often changes dynamically. To alleviate this problem, we propose a new vertical federation learning method, DVFL, which adapts to dynamic data distribution changes through knowledge distillation. In DVFL, most of the computations are held locally to improve data security and model efficiency. Our extensive experimental results show that DVFL can not only obtain results close to existing VFL methods in static scenes, but also adapt to changes in data distribution in dynamic scenarios.

==> Method.tex <==
\section{Method}
%\subsection{Overview}
In this section, we will describe the model of Dynamic Vertical Federated Learning (DVFL) in detail. The goal of DVFL is to improve the performance of the model by using the data of party A and party B in the context of data privacy protection. DVFL has 4 modules, namely representation encoding module, representation estimation module, estimation correction module, and classification module. The description of each module is as follows.


\subsection{Representation Encoding}
Firstly, we use neural networks to encode the feature representation from the raw data. Let $\mathbf{r}^p = h^p (\mathbf{x}^p)$ represents the feature representation of raw data $\mathbf{x}^p$ though neural network $h^p$, where party $p \in \{A, B\}$, $\mathbf{r}^p \in \mathbb{R}^{N^p \times d^p}$, $d^p$ is the dimension of the top hidden representation layer of neural networks in party $p$, and $N^p$ is the number of examples in party $p$. We use an auto-encoder model to get $h^p$. An auto-encoder has an encoder function $h^p$ and a decoder function $\widetilde{h}^p$.

In the encoding process, the input sample $\mathbf{x}^p$ is mapped to the feature space $\mathbf{r}^p$ through encoder $h^p$
\begin{equation}
\mathbf{r}^p = h^p(\mathbf{x}^p)
\end{equation}
% \begin{equation}
%     h^p(x) = W^p x + b^p
% \end{equation}

In the decoding process, the feature representation $r^p$ is mapped back to the original space through decoder $\widetilde{h}^p$ to obtain the reconstructed sample
\begin{equation}
\bar{\mathbf{x}}^p = \bar{h}^p(\mathbf{r}^p)
\end{equation}

The loss of the auto-encoder is 
\begin{equation}
\mathcal{L}_{AE}^P = \frac{1}{N^p} \sum_{i=1}^{N^p} ||\textbf{x}_i^p - \bar{\textbf{x}}_i^p||_F^2
\end{equation}
where $N^p$ is the number of samples in party p.

$h^p$ and $\bar{h}^p$ are implemented by two independent multi-layer perceptions. The parameters of $h^p$ and $\bar{h}^p$ are optimized by minimizing $\mathcal{L}_{AE}^P$ via stochastic gradient descent (SGD). The training of $h^p$ is unsupervised and completed locally in party $p$.

%so there is no risk of data leakage in this part.  


\subsection{Representation Estimation of Missing Feature}
% Build upon the encoded feature representations,
Similar to \cite{DBLP:journals/corr/abs-2008-10838}, we estimate representations for the missing features in party A by transfer learning. 

We propose a Representation Estimation Networks (REN). Given the feature representation $\mathbf{r}^A$, REN generates the estimate representations of $\mathbf{r}^B$ by
\begin{equation}
\widetilde{\mathbf{r}}^B = g^B (\mathbf{r}^A)
\end{equation} 
where $\widetilde{\mathbf{r}}^B$ is the estimate representation of $\mathbf{r}^B$ based on $\textbf{r}^A$, and $g^B$ is the REN implemented by a neural network

Let $\mathcal{D}_{ov,0}^A$ denote the overlapping example in $\mathcal{D}^A$ and $\mathcal{D}_0^B$, the parameters of REN are trained based on $\mathcal{D}_{ov,0}^A$ and $\mathcal{D}_0^B$. The loss function of REN is 
\begin{equation}
\mathcal{L}_{REN} = \frac{1}{N_0^B} \sum_{i=1}^{N_0^B} ||\mathbf{r}_{i,0}^{B} - \widetilde{\mathbf{r}}_{i,0}^{B}||_F^2
\end{equation}
where $\mathbf{r}_{i,0}^{B}$ is the i-th sample at timestamp $t = 0$ in party B, $N_0^B$ is the size of $\mathcal{D}_0^B$ ($|\mathcal{D}_0^B| = |\mathcal{D}_{ov,0}^A|$)

We use $\Theta_B$ to denote the model parameters of $g^B$. In the process of optimizing $\Theta_B$ with mini-batch SGD, we need to obtain the gradient $\nabla \mathcal{L}_{REN}$ in the training of each batch. According to the chain rule in back-propagation, we can obtain the gradient of $\Theta_B$ by:
\begin{equation}
\label{eq_Backpro_REN}
\nabla \mathcal{L}_{REN}(\Theta_B) = \frac{\partial \mathcal{L}_{REN}}{\partial \widetilde{\mathbf{r}}^B} \cdot \frac{\partial \widetilde{\mathbf{r}}^B}{\partial \Theta_B}
\end{equation}

Specifically, we divide $\mathcal{D}_0^A$ into $n$ batches, and each batch has $m$ items. For the set of the $j$-th batch $\mathcal{D}_{0,j}^A = \{x_i\}_{i=j \times m}^{(j+1) \times m}$, we obtain the gradient $\nabla \mathcal{L}_{REN}(\Theta_B^j)$ through the following steps

\begin{enumerate}
\item Party A computes the estimated representations $E_{0,j}^B = \{\widetilde{\mathbf{r}}_i^B\}_{i=j \times m}^{(j+1) \times m}$ based on current $\Theta_B$ and send $E_{0,j}^B$ to party B; 
\item Party B computes the gradient $\frac{\partial \mathcal{L}_{REN}}{\partial \widetilde{\mathbf{r}}^B}$, then encrypts the gradient with Homomorphic Encryption (HE) and send to party A; 
\item Note that so far, the encrypted gradient $[[\frac{\partial \mathcal{L}_{REN}}{\partial \widetilde{\mathbf{r}}^B}]]$ is the gradient for $\widetilde{r}^B$, we need to obtain the gradient $\nabla \mathcal{L}_{REN}(\Theta_B^j)$ by Eq. \ref{eq_Backpro_REN}. In party A, we can obtain $\frac{\partial \widetilde{\mathbf{\mathbf{r}}}^B}{\partial \Theta_B}$. Then according to the properties of HE and the chain rule, we can obtain the encrypted gradient $[[\nabla \mathcal{L}_{REN}(\Theta_B^j)]]$ by multiplying $\frac{\partial \widetilde{\mathbf{r}}^B}{\partial \Theta_B}$ and $[[\frac{\partial \mathcal{L}_{REN}}{\partial \widetilde{\mathbf{r}}^B}]]$; 
\item Since party B holds the key of the encryption, party A sends $[[\nabla \mathcal{L}_{REN}(\Theta_B^j)]]$ to party B, then party B sends back $\nabla \mathcal{L}_{REN}(\Theta_B^j)$ to party A after decryption. 
\end{enumerate}

After obtaining the gradient, the model parameters are updated as follows:
\begin{equation}
\Theta_B^{j+1} = \Theta_B^j - \eta \nabla \mathcal{L}_{REN}(\Theta_B) 
\end{equation}
where $\eta$ is the learning rate.

The detailed process of training the representation estimation network is in Fig. \ref{fig_LEN}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/REN.pdf}
    \caption{Process of REN parameters update}
\label{fig_LEN}
\end{figure} 

\subsection{Estimated Representation Correction}
Then, we train a perturbation generator that create perturbations to correct the estimated representation $\widetilde{\mathbf{r}}_i^B$. To define the perturbation, we need to know two issues: 1) where to perturb and 2) how to determine the perturbation magnitude. Thus, we factorize the  perturbation as
\begin{equation}
\epsilon = \delta \odot p
\end{equation}
where $\delta \in \mathbb{R}$ is a magnitude and $\delta$ is a user-defined parameter. $c \in \{0, 1\}^N$ denotes the vector of perturbed dimensions, and $\odot$ represents element-wise product.

The vector of perturbed dimensions of $\widetilde{\mathbf{r}}^B$ is
\begin{equation}
%p = I(g_p(\mathbf{r}^B - \widetilde{\mathbf{r}}^B))
p = I(g_p(\widetilde{\mathbf{r}}^B))
\end{equation}
where $g_p$ is implemented by a neural network, and $I$ is an indicator 
\begin{equation}\label{equ:f}
I(x)=
\begin{cases}
-1& x<-0.5\\
0& -0.5\leq x\leq 0.5\\
1& x>0.5
\end{cases}
\end{equation}

The corrected representation is
\begin{equation}
\hat{\mathbf{r}}^B = \widetilde{\mathbf{r}}^B + \epsilon
\end{equation}

The loss function of $g_p$ is:
\begin{equation}
\mathcal{L}_{p} = \frac{1}{N_0^B} \sum_{i=1}^{N_0^B} ||\mathbf{r}_i^B - \hat{\mathbf{r}}_i^B||_F^2
\end{equation}
where $N_0^B = |\mathcal{D}_0^B|$

The parameters of $g_p$ is trained by minimizing $\mathcal{L}_p$ with mini-batch SGD. 

\subsection{Classifier}
\begin{figure}[ht]
\label{fig_dis}
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/Distill.pdf}
    \caption{Process of training classifier}
\end{figure} 

Then, the overall representation of $\mathbf{x}$ is
\begin{equation}
\mathbf{r} = \mathbf{r}^A \oplus \hat{\mathbf{r}}^B
\end{equation}
where $\oplus$ denotes concatenate operation.

We use a neural network model $f_{c,t}$ as the classifier at timestamp $t$. According to our problem setting, the classifier should be applicable to dynamic vertical federated learning, i.e., the size of $\mathcal{D}^B$ increase with time, and the data distribution of $\bigtriangleup \mathcal{D}_t^{B}$ is not necessarily the same as that of $\mathcal{D}_{t-1}^B$. 

Intuitively, we can use the fine-tuning technique to update the model parameters in dynamic vertical federated learning. But fine-tuning is mainly applicable to the situation where the data distribution is unchanged. When the data distribution in $\bigtriangleup \mathcal{D}_t^B$ and $\mathcal{D}_{t-1}^B$ is quite different, the problem of catastrophic forgetting will occur, which makes the trained classifier is biased towards the data distribution of $\bigtriangleup D_{t}^B$. We solve the problem by distilling the well-trained model at the previous timestamp\cite{DBLP:conf/iclr/LiJZKD21,DBLP:journals/pami/LiH18a}. The new model is learned by using a distilling loss and a classification loss.

Let $\mathcal{D}_{ov,t}^A$ be the overlapping examples between $\mathcal{D}^A$ and  $\mathcal{D}_t^B$, $\bigtriangleup \mathcal{D}_{ov,t}^A$ be the overlapping examples between $\mathcal{D}^A$ and $\bigtriangleup \mathcal{D}_t^B$, $N_{ov,t}^A = |\bigtriangleup \mathcal{D}_{ov,t}^A|$, and the distilling loss is formulated as follows:
\begin{equation}
    \mathcal{L}_{d,t} = - \sum_{i=1}^{N_{ov,t}^A} \sum_{c=1}^C  \frac{e^{\hat{y}_{i, t-1}^c/F}}{\sum_{j=1}^C e^{\hat{y}_{i, t-1}^j/F}} log \frac{e^{\hat{y}_{i,t}^c}/F}{\sum_{j=1}^C e^{\hat{y}_{i,t}^j/F}} 
\end{equation}
where $C$ is the number of classes in $\bigtriangleup \mathcal{D}_{ov,t}^A$, $\hat{y}^{i,t}_c$ is the $c$-th element in the result of predicting $\mathbf{x}_i$ based on $\Theta_{t}$, and $F$ is the temperature scalar. We set $F = 2$ in our experiment.  

We use cross entropy to compute the classification loss:
\begin{equation}
\mathcal{L}_{c,t} = - \sum_{i=1}^{N_{ov,t}^A}\sum_{c=1}^{C} w_c y_{i,t}^c log (\hat{y}_{i,t}^c)
\end{equation}
where $w_c$ is the weight of class $c$. $w_c = 1$ for balanced dataset.

The overall loss combines the distilling loss and the classification loss:
\begin{equation}
\mathcal{L}_t = \lambda \mathcal{L}_{d,t} + (1-\lambda) \mathcal{L}_{c,t}, 
\end{equation} 
where the parameter $\lambda$ is used to balance the two terms. 

Then, we can train $f_{c,t}$ by minimize $\mathcal{L}$ via SGD. The training process is held in party A.

\subsection{Security and Privacy Analysis}
In terms of privacy-preserving, the training of DVFL satisfies the following restrictions:
\begin{enumerate} 
\item DVFL does not require parties to share their original data and model parameters
\item Only intermediate representation and gradients are exchanged. 
\item Unlike previous studies (e.g., \cite{DBLP:journals/corr/abs-2008-10838} \cite{DBLP:journals/corr/abs-1812-03337}) that use a single neural network to encode the original feature as an intermediate representation, the intermediate representation participating in the exchange in our model is the result of the original feature encoded by multiple heterogeneous neural networks. This further strengthens the security of the algorithm.
\item The exchange of the gradients will not expose the model parameters or local data.
\end{enumerate}

DVFL consists of 4 modules. We proof DVFL meets the restrictions by analyzing the data security of each module.

\textbf{Representation Encoding Module.} In this module, party A and party B use local data to train their own auto-encoders. All training is conducted locally and does not involve data sharing between parties.

\textbf{Representation Estimation Module.} The data exchanges in this module are: 1) The estimated representation $\widetilde{\mathbf{r}}^B$ generated by party A will be sent to party B; 2) The encrypted gradient $[[\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B}]]$ and the decrypted gradient $\nabla \mathcal{L}_{REN}(\Theta_B)$ will be sent from party B to party A, and the encrypted gradient $[[\nabla \mathcal{L}_{REN}(\Theta_B)]]$ will be sent from party A to party B. 

Firstly, sending the estimated representation $\widetilde{\mathbf{r}}^B$ from party A to party B satisfies the restrictions. Since $\widetilde{\mathbf{r}}^B = g^B(h^A(\mathbf{x}^A))$, $g^B$ and $h^A$ are two neural networks with different structures, $\widetilde{\mathbf{r}}^B$ is the result of the original feature encoded by multiple heterogeneous neural networks. 

Secondly, in the exchange of the gradients, even the encoded representation $\mathbf{r}^A$ and $\mathbf{r}^B$ are not inferrable by each other under certain constraints. When $[[\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B}]]$ is sent to party A, the gradient is encrypted, and A cannot obtain the gradient without the key stored in party B. When party B gets $[[\nabla \mathcal{L}_{REN}(\Theta_B)]]$, party B cannot infer the data or model in party A since party B do not know the network structure of $\Theta_B$. When party A get the decrypted $\nabla \mathcal{L}_{REN}(\Theta_B)$, $\mathbf{r}^B$ is not inferrable by party A when $|\Theta_B| < m \times d^B$, where $|\Theta_B|$ is the number of parameters of $g^B$, $m$ is the batch size, and $d^B$ is the length of $\mathbf{r}^B$. The only possible way to infer $\mathbf{r}^B$ by party A is to obtain $\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B}$, and then we have the following claim:

\textbf{Claim 1.} \textit{Party A cannot infer $\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B}$ when $|\Theta_B| < m \times d^B$}.

\textit{Proof.} Recall that $\nabla L_{REN} (\Theta_B) = \frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B} \frac{\partial \widetilde{\mathbf{r}}^B}{\partial \Theta_B}$, party A can obtain $\nabla L_{REN} (\Theta_B)$ and $\frac{\partial \widetilde{\mathbf{r}}^B}{\partial \Theta_B}$ in each batch of training. To get $\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}^B}$, party A need to solve the linear equation group:
\begin{equation}\label{equ:leg}
\begin{cases}
\begin{aligned}
\nabla \mathcal{L}_{REN}(\Theta_{B(1)})&= \frac{1}{m} \sum_{i=1}^{m} \sum_{j=1}^{d^B} \frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}_{i(j)}^B} \frac{\partial \widetilde{\mathbf{r}}_{i(j)}^B}{\partial \Theta_{B(1)}}\\
\nabla \mathcal{L}_{REN}(\Theta_{B(2)})&= \frac{1}{m} \sum_{i=1}^{m} \sum_{j=1}^{d^B} \frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}_{i(j)}^B} \frac{\partial \widetilde{\mathbf{r}}_{i(j)}^B}{\partial \Theta_{B(2)}}\\
&\vdots \\
\nabla \mathcal{L}_{REN}(\Theta_{B(K)})&= \frac{1}{m} \sum_{i=1}^{m} \sum_{j=1}^{d^B} \frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}_{i(j)}^B} \frac{\partial \widetilde{\mathbf{r}}_{i(j)}^B}{\partial \Theta_{B(K)}}\\
\end{aligned}
\end{cases}
\end{equation}
where $\Theta_{B(i)}$ is the i-th parameter in $\Theta_B$, $\widetilde{\mathbf{r}}_i(j)^B$ is the value of the j-th dimension in the representation of the i-th item in the batch.  

In this case, the number of equations is $K = |\Theta_B|$ and the number of parameters is $m \times d^B$. When  $|\Theta_B| < m \times d^B$, there are infinite different solutions of $\frac{\partial L_{REN}}{\partial \widetilde{\mathbf{r}}_{i(j)}^B}$ ($1 < i < m$, $1 < j < d^B$). Thus, the claim is proofed.

\textbf{Estimation Correction Module.} In this module, the estimated representation $\widetilde{\mathbf{r}}^B$ generated by party A will be sent to party B, and the perturbation $\epsilon$ generated by party B will be sent to party A. As discussed above, sending $\widetilde{\mathbf{r}}^B$ to party B satisfies the restrictions. Since $\epsilon = I(g_p(g^B(\mathbf{r}^A)))$, $g_p$ and $g^B$ are neural networks of different structures, sending $\epsilon$ to party A satisfies the restrictions.

\textbf{Classification Module.} In this module, the classifier is trained locally in party A, and there is no risk of data leakage.

Thus, each step in DVFL satisfies the restrictions, and the model is considered secure in this case \cite{DBLP:journals/corr/abs-1812-03337,DBLP:journals/corr/abs-2008-10838}. 
